Style Modeling for Multi-Speaker Articulation-to-Speech

In this paper, we propose a neural articulation-to-speech (ATS) framework that synthesizes high-quality speech from articulatory signal in a multi-speaker situation. Most conventional ATS approaches only focus on modeling contextual information of speech from a single speaker's articulatory features. To explicitly represent each speaker's speaking style as well as the contextual information, our proposed model estimates style embeddings, guided from the essential speech style attributes such as pitch and energy. We adopt convolutional layers and transformer-based attention layers for our model to fully utilize both local and global information of articulatory signals, measured by electromagnetic articulography (EMA). Our model significantly improves the quality of synthesized speech compared to the baseline in terms of objective and subjective measurements in the Haskins dataset.

==> introduction_1014backup_.tex <==
\section{Introduction}
\label{sec:intro}




%1.1 ats의 정의 및 input 설명 간단히

%1.2 기존의 ats연구흐름 (1. rule-based --> directly & two stages 2)deep-learning 연구-->deep learning-based ats 구조 간략히)

% However 대부분은 single speaker에대한 approch가 많다. (포괄적으로)
% 1.3 multi-speaker ATS에 대한 필요성 & 어려움 

% 1.3.1 multi-speaker ATS에 대한 필요성 구체적 나열


% 1.3.2 multi-speaker ATS의 어려움 (각자의 spk에 대한 특징을 ema로 부터 추정하기 힘들다)

% 1.4 Proposed Model

    







% Definition or ATS
% Why ATS is needed
% What is EMA signal meaning?!?!
% Previous approaches
    % statistical
    % deep-learning based
    % data shortage
    % intermediate feature extraction
    % directly extract speech from dataset
    % use not public dataset
    % Contribution
        % Proposed 
    
\if
% (leeji) 내용 흐름 초안
% ATS란 이런 것이다. 이런 곳에 쓸 수 있다.
% 일반적으로 어떤 articulatory feature를 speech production에 사용하는가, 그 중에서 EMA를 강조
% EMA-to-speech의 기존 접근법, 그 방법들의 limitation 간략히 설명 - single-speaker임을 강조
%       근데 굳이 multispeaker여야 하는지 태클 걸릴 수 있음 (한 사람에 대해서만 해도 되는 게 아닌가?) -> 일반적으로 multi-speaker 보다 speaker dependent한 모델성능이 좋음.
%       각각의 speaker에 대해서 다른 모델들을 만들면 cost가 너무 많이 든다.    
%       별도의 fine-tuning 없이 다양한 사람에게 적용 가능하다는 것을 언급하기?
% 나는 ATS 논문을 많이 안 읽어봤으므로 다른 논문 intro도 보면서 이상한 거 있으면 수정하세여 (thank you for your nice introduction~)



% ===== Definition of SSI & necessity of this technologies =====
Silent speech interface (SSI) \cite{denby2010silent, freitas2017introduction} is an emerging technology that is designed to identify phonetic information or to generate speech signals from non-auditory sources.

Recently, SSI is getting a great deal of public attention because it is a useful communication technology for social conventions. 
It is also an alternative way of speech communication for patients who experience inconvenience in speech production.
Among many different types of SSI, an articulation-to-speech (ATS) system has gained popularity because it is able to synthesize intelligible speech.
%For example, laryngetomees, who underwent an surgery of removing their larynx, cannot properly produce audible speech. 
%As a solution, an articulation-to-speech (ATS) algorithm can be designed to synthesize intelligible speech from articulatory movements.
% leeji: 아래 사례도 쓸거라면 앞 내용만큼 쓰든지 아예 빼는 게 흐름이 깔끔할 듯함
%For highly noise clustered background like inside the bus, SSI can also effectively transfer a human's word to others.



% ==== Introduction to non-auditory sources and their representations ====
Articulatory movements are represented in various ways depending on the placement of articulators and types of sensors needed for estimating the movements.
Commonly used representations include surface electromyography (sEMG), permanent magnetic articulography (PMA), ultrasound tongue imaging (UTI) and electromagnetic midsagittal articulography (EMA or EMMA). 
EMA \cite{hoole1999electromagnetic} measures and records kinematic movements of articulators such as lips, tongue, jaw, and velum using low field-strength electromagnetic fields.
Since EMA detects the movements of the most important articulators for speech intelligibility, it is one of the most frequently chosen input representations to design an ATS system.
In our approach, we also utilize EMA signal as the input of our proposed model.


% ===== Articulatory to acoustic (overall) =====
% leeji: 이 부분 서술을 단정적으로 쓰기 좀 애매한데, related work와 비교해서 수정하기
% EMA-to-speech 논문들만 넣으면 좋겠지만, 여의치 않을 경우 맥락에만 맞으면 ATS 논문으로 넣기
% leeji: non-deep learning methods 중 다음 비워놓은 곳에 해당되는 single-speaker 논문이 있으면 추가
% non-deep learning method 중 waveform 으로 바로 바꾸는 논문이 있으면 이대로 두고,
Some ATS algorithms directly synthesize speech waveforms from articulatory movements~\cite{sondhi1987hybrid}. Other approaches take two step approaches; they first convert articulatory inputs to acoustics features such as linear spectrogram~\cite{toda2004mapping} or other acoustic features~\cite{kaburagi1998determination, hueber2011statistical}, then synthesize speech waveforms from the acoustic features. 
% Kang: include ref. more
Recently, deep learning-based approach~\cite{gaddy2021improved} is gaining a lot of popularity due to its high performance compared to conventional rule-based methods.
However, to the best of our knowledge, these approaches are confined to a single speaker system.
To extend its applicability and generalization capability, the ATS model needs to support multi-speaker cases, too.



% =====  Contribution of proposed method =====
% Kang: contribution을 잘 정리해서 포함할 것
% Kang: 더 자세히 서술 필요.
In this paper, we propose a multi-speaker ATS framework that synthesizes high-quality speech signal from articulatory movements. From the assumption that EMA signals have context information and speech style characteristics, our approach directly constructs style vector from EMA input data. Since the framework is designed to combine convolution and transformer layer, both of local and global information is effectively captured. 
Our paper is organized as follows. In section \ref{sec:Related works}, we summarize previous approaches that are related with our proposed model. In section \ref{sec:proposed_model}, we describe our proposed model in detail. In Section
\ref{sec:experiments}, we show experimental results that verify the superior performance of our model. Finally, Section \ref{sec:conclusion} provides our conclusions.

\fi

\begin{figure*}[htb]
\label{proposed_model}
\centering
\centerline{\includegraphics[width=15cm]{img/proposed_new.png}}
\caption{Overall framework of the proposed model. Our system is trained with a two-step approach ((a) to (b)). %Each step is trained separately. 
(c) depicts the diagram of the inference stage. 
(a): mel encoder, mel decoder and mel generator are trained jointly. (b): Only EMA encoder is trained to make style embedding from combined EMA vector with speaker embedding. (c): Mel encoder is replaced from EMA encoder, so model can directly generate acoustic featurs from input EMA signal only.}   
\end{figure*}






